Computationally Efficient Technique for Nonlinear Poisson-Boltzmann Equation

Discretization of non-linear Poisson-Boltzmann Equation equations results in a system of non-linear equations with symmetric Jacobian. The Newton algorithm is the most useful tool for solving non-linear equations. It consists of solving a series of linear system of equations (Jacobian system). In this article, we adaptively define the tolerance of the Jacobian systems. Numerical experiment shows that compared to the traditional method our approach can save a substantial amount of computational work. The presented algorithm can be easily incorporated in existing simulators.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, ps, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a ps file, type "make ps".
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# Rouben Rostmaian
# September 2002

TEXFILE =   article.tex
#TEXFILE	= slides.texTPFA_diagonal_perm_variable.tex

.PHONY: dvi ps pdf clean

pdf:	$(TEXFILE:.tex=.pdf)
ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	( \
	\latex $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)

%.ps: %.dvi
	\dvips -q -t a4 $<

%.pdf: %.ps
	\ps2pdf -dPDFSETTINGS=/prepress $<

clean:
	@\rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.ps)

